Origin of Jumping Oscillons in an Excitable Reaction-Diffusion System

Oscillons, i.e., immobile spatially localized but temporally oscillating structures, are the subject of intense study since their discovery in Faraday wave experiments. However, oscillons can also disappear and reappear at a shifted spatial location, becoming jumping oscillons (JOs). We explain here the origin of this behavior in a three-variable reaction-diffusion system via numerical continuation and bifurcation theory, and show that JOs are created via a modulational instability of excitable traveling pulses (TPs). We also reveal the presence of bound states of JOs and TPs and patches of such states (including jumping periodic patterns) and determine their stability. This rich multiplicity of spatiotemporal states lends itself to information and storage handling.

==> ghtikz.tex <==
\usetikzlibrary{arrows.meta}
\tikzset{%
  >={Latex[width=1mm,length=3mm]},
% Specifications for style of nodes:
base/.style = {rectangle, rounded corners, draw=black,
                minimum width=3mm, minimum height=1mm,
%               text width=30mm, 
align=left},%, font=\sffamily},  
le/.style = {rectangle, rounded corners, draw=black,  
      minimum width=3mm, minimum height=5mm, %text width=10mm,  
align=left},
mi/.style = {rectangle, rounded corners, draw=black, % minimum width=3cm, 
    minimum height=2mm, %text width=32mm,  
align=left}, 
sm/.style = {draw=black, rounded corners, align=left},
ri/.style = {draw=black, rounded corners}
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

